CG-Net: Conditional GIS-aware Network for Individual Building Segmentation in VHR SAR Images

Object retrieval and reconstruction from very high resolution (VHR) synthetic aperture radar (SAR) images are of great importance for urban SAR applications, yet highly challenging owing to the complexity of SAR data. This paper addresses the issue of individual building segmentation from a single VHR SAR image in large-scale urban areas. To achieve this, we introduce building footprints from GIS data as complementary information and propose a novel conditional GIS-aware network (CG-Net). The proposed model learns multi-level visual features and employs building footprints to normalize the features for predicting building masks in the SAR image. We validate our method using a high resolution spotlight TerraSAR-X image collected over Berlin. Experimental results show that the proposed CG-Net effectively brings improvements with variant backbones. We further compare two representations of building footprints, namely complete building footprints and sensor-visible footprint segments, for our task, and conclude that the use of the former leads to better segmentation results. Moreover, we investigate the impact of inaccurate GIS data on our CG-Net, and this study shows that CG-Net is robust against positioning errors in GIS data. In addition, we propose an approach of ground truth generation of buildings from an accurate digital elevation model (DEM), which can be used to generate large-scale SAR image datasets. The segmentation results can be applied to reconstruct 3D building models at level-of-detail (LoD) 1, which is demonstrated in our experiments.

==> bio.tex <==
% ******** bio ************%
\begin{IEEEbiography}{Yao Sun}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Yuansheng Hua}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Lichao Mou}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Xiao Xiang Zhu}
Biography text here.
\end{IEEEbiography}

==> sections/secF_w_wo_error.tex <==

\begin{figure}[!]
    \centering
    \settoheight{\tempdima}{\includegraphics[width=.15\textwidth]{figs/secF/06701_0.png}}%
    \begin{tabularx}{0.99\linewidth}{C@{\hskip2pt}C@{\hskip2pt}C@{\hskip2pt}C@{\hskip2pt}}
    \\\vspace{-0.4cm}
    \textbf{\hspace{0.3cm}\footnotesize{b1}} &\textbf{\footnotesize{b2}}& \textbf{\footnotesize{b3}}
    \\\vspace{-0.4cm}
    \rowname{\footnotesize{SAR image}}
    \hspace{-0.06cm}
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/00070_0.png}}}& 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06701_0.png}}}&
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06101_0.png}}}&
    \\\vspace{-0.4cm}
    \rowname{\hspace{-0.3cm}\footnotesize{CBF}} 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/00070_1.png}}}& 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06701_1.png}}}&
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06101_1.png}}}&
    \\\vspace{-0.4cm}
    \rowname{\hspace{-0.3cm}\footnotesize{GT}}
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/00070_3_gt.png}}}& 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06701_3_gt.png}}}&
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06101_3_gt.png}}}&
    \\\vspace{-0.4cm}
    \rowname{\hspace{-0.3cm}\footnotesize{CBF Prediction}} 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/00070_4_correct.png}}}& 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06701_4_correct.png}}}&
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06101_4_correct.png}}}&
    \\\vspace{-0.4cm}
    \rowname{\hspace{-0.3cm}\footnotesize{CBF-E Prediction}} 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/00070_5_error.png}}}& 
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06701_5_error.png}}}&
    \subfloat{{\includegraphics[width=.13\textwidth]{figs/secF/06101_5_error.png}}}&
    & & & &\\
    \end{tabularx}
    \caption{Examples of segmentation results of networks trained using complete building footprints (abbreviated as CBF) and networks trained using building footprints with positioning errors (abbreviated as CBF-E). }
    \label{fig:cbf_cbfe}
\end{figure}

==> sections/subfig/gisF_subfig.tex <==

\begin{figure*}
    \centering
    \begin{tabularx}{0.95\linewidth}{@{}c@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}}
    \\\vspace{-0.35cm}
    \textbf{SAR image} & \textbf{GISF} & \textbf{GT} & \textbf{FCN} & \textbf{FCN+CG} & \textbf{DeepLabV3} & \textbf{DeeplabV3+CG}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_08.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_08.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_12.png}}}\\
    \end{tabularx}
    \caption{Examples of segmentation results for the GISF dataset. }
    \label{fig:subgisF}
\end{figure*}

==> sections/subfig/gisF_w_ref.tex <==
\newlength{\tempdima}
\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\tempdima][c]{\textbf{#1}}}}


\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}


\begin{figure*}
    \settoheight{\tempdima}{\includegraphics[width=.11\textwidth]{figs/subfigs/00554_00.png}}%
    \centering
    \begin{tabularx}{0.98\linewidth}{@{}c@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}}
    \\\vspace{-0.35cm}
    & \textbf{ref} & \textbf{SAR image} & \textbf{GISF} & \textbf{GT} & \textbf{FCN} & \textbf{FCN+CG} & \textbf{DeepLabV3} & \textbf{DeeplabV3+CG}
    \\\vspace{-0.4cm}
    \rowname{B 1} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_08.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_12.png}}
    \\\vspace{-0.4cm}
    \rowname{B 2} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_00.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_01.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_08.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_07.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_12.png}}
    \\\vspace{-0.4cm}
    \rowname{B 3} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_00.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_01.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_08.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_12.png}}
    \\\vspace{-0.4cm}
    \rowname{B 4} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_00.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_01.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_08.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_07.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_12.png}}
    \\\vspace{-0.4cm}
    \rowname{B 5} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_08.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_12.png}}
    \\\vspace{-0.4cm}
    \rowname{B 6} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_00.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_01.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_08.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_07.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_12.png}}
    \\\vspace{-0.4cm}
    \rowname{B 7} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_00.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_01.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_08.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_07.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_12.png}}
    \\\vspace{-0.4cm}   
    \rowname{B 8} &
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_00.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_01.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_08.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_07.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_09.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_10.png}}& 
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_11.png}}& \hspace{-0.45cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_12.png}}\\
    \end{tabularx}
    \caption{Examples of segmentation results: GISF}
    \label{fig:sub2}
\end{figure*}

==> sections/subfig/gisFpatch.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics{patches GISF}
%     \caption{Examples of segmentation results on patches: GISF}
%     \label{fig:pgisF}
% \end{figure*}



\begin{figure*}[h!]
    \centering
    \begin{tabularx}{0.95\linewidth}{@{}c@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}}
    \\\vspace{-0.35cm}
    \textbf{SAR image} & \textbf{GISV} & \textbf{GT} & \textbf{FCN} & \textbf{FCN+CG} & \textbf{DeepLabV3} & \textbf{DeeplabV3+CG}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_12.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_09.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_10.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_11.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_12.png}}}
    % \\\vspace{-0.4cm}
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_01.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_02.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_07.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_09.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_10.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_11.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_12.png}}}
    % \\\vspace{-0.4cm}
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_01.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_02.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_07.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_09.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_10.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_11.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_12.png}}}
    \\
    & & & & & & &\\
    \end{tabularx}
    \caption{Examples of segmentation results on patches for the GISF dataset. }
    \label{fig:pgisF}
\end{figure*}

==> sections/subfig/gisV_subfig.tex <==

\begin{figure*}
    \centering
    \begin{tabularx}{0.95\linewidth}{C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}}
    \\\vspace{-0.35cm}
    \textbf{SAR image} & \textbf{GISV} & \textbf{GT} & \textbf{FCN} & \textbf{FCN+CG} & \textbf{DeepLabV3} & \textbf{DeeplabV3+CG}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00554_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00524_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00590_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10589_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/02539_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00515_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/00313_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_02.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_03.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_04.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_05.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/subfigs/10586_06.png}}}\\
    & & & & & &\\
    \end{tabularx}
    \caption{Examples of segmentation results for the GISV dataset. }
    \label{fig:subgisV}
\end{figure*}

==> sections/subfig/gisV_w_ref.tex <==
\newlength{\tempdima}
\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\tempdima][c]{\textbf{#1}}}}


\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}


\begin{figure*}
    \centering
    \begin{tabularx}{0.98\linewidth}{C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}}
    \\\vspace{-0.35cm}
    \textbf{ref} & \textbf{SAR image} & \textbf{GISV} & \textbf{GT} & \textbf{FCN} & \textbf{FCN+CG} & \textbf{DeepLabV3} & \textbf{DeeplabV3+CG}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00554_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00590_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00515_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10589_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00313_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/02539_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/00524_06.png}}
    \\\vspace{-0.4cm}
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_00.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_01.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_02.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_07.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_03.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_04.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_05.png}}&
    \subfloat{\includegraphics[width=.115\textwidth]{figs/subfigs/10586_06.png}}\\
    & & & & & &\\
    \end{tabularx}
    \caption{Examples of segmentation results: GISV}
    \label{fig:sub2}
\end{figure*}

==> sections/subfig/gisVpatch.tex <==


% \begin{figure*}
%     \centering
%     \includegraphics{patches GISV}
%     \caption{Examples of segmentation results on patches: GISV}
%     \label{fig:pGISV}
% \end{figure*}


\begin{figure*}[h!]
    \centering
    \begin{tabularx}{0.95\linewidth}{@{}c@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}C@{\hskip1pt}}
    \\\vspace{-0.35cm}
    \textbf{SAR image} & \textbf{GISF} & \textbf{GT} & \textbf{FCN} & \textbf{FCN+CG} & \textbf{DeepLabV3} & \textbf{DeeplabV3+CG}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_01.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_07.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_03.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_04.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_05.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00530_06.png}}}
    \\\vspace{-0.4cm}
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_01.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_08.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_07.png}}}&
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_03.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_04.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_05.png}}}& 
    \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00501_06.png}}}
    % \\\vspace{-0.4cm}
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_01.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_08.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_07.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_03.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_04.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_05.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00003_06.png}}}
    % \\\vspace{-0.4cm}
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_01.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_08.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_07.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_09.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_10.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_11.png}}}& 
    % \subfloat{\reflectbox{\includegraphics[width=.13\textwidth]{figs/patches/00004_12.png}}}
    \\
    & & & & & & &\\
    \end{tabularx}
    \caption{Examples of segmentation results on patches for the GISV dataset. }
    \label{fig:pgisV}
\end{figure*}


